Hold 'em and Fold 'em: Towards Human-scale, Feedback-Controlled Soft Origami Robots

An underdeveloped capability in soft robotics is proprioceptive feedback control, where soft actuators can be sensed and controlled using only sensors on the robot's body. Additionally, soft actuators are often unable to support human-scale loads due to the extremely compliant materials in use. Developing both feedback control and the ability to actuate under large loads (e.g. 500 N) are key capacities required to move soft robotics into everyday applications. In this work, we independently demonstrate these key factors towards controlling and actuating human-scale loads: proprioceptive (embodied) feedback control of a soft, pneumatically-actuated origami robot; and actuation of these origami origami robots under a person's weight in an open-loop configuration. In both demonstrations, the actuators are controlled by internal fluidic pressure. Capacitive sensors patterned onto the robot provide position estimation and serve as input to a feedback controller. We demonstrate position control of a single actuator during stepped setpoints and sinusoidal trajectory following, with root mean square error (RMSE) below 4 mm. We also showcase the actuator's potential towards human-scale robotics as an "origami balance board" by joining three actuators into an open-loop controlled system with a platform that varies its height, roll, and pitch. This work contributes to the field of soft robotics by demonstrating closed-loop feedback position control without visual tracking as an input and lightweight, soft actuators that can support a person's weight. The project repository, including videos, CAD files, and ROS code, is available at https://parses-lab.github.io/kresling_control.

==> judging.tex <==
Judging Criteria

The judging criteria listed below will be used to determine the winners of the Summer 2023 Soft Robotic Toolkit competition for each of the listed categories. Each project submitted will receive a score from 1-10 in the three below categories. The submissions with the highest combined score across all three of the judging criterias will be selected as the winners.

Innovative Design (10 points)
The authors have shown that there is a clear need for this design
The submission is state of the art in the soft robotic field
The authors use a creative approach to solve a real world challenge and have shown that there is a need for their design
The submission has the potential to progress the soft robotic field in a meaningful way
Presentation and User Considerations (20 points)
The submission has a high quality of Implementation. Did the team build a working prototype? Does the prototype meet the functional requirements set by the team? 
Care and consideration have been taken for the aesthetic presentation of the design submission
The authors have paid attention to the usability and accessibility of the design (how widely can this design be potentially used)
Does this design require fully custom components, or are barriers to entry lowered such that other users will more rapidly be able to adopt the design
Well-Documented Project (20 points)
Submission guidelines were followed and all required sections are included as written
The design process is easily understood to a general audience
The submission documentation clearly lays out each step in the fabrication and demonstration process
The design is able to be replicated based on the documentation provided


==> ral_paper.tex <==
\begin{abstract}
As soft roboticists further investigate approaches to position or force feedback control, accurate and embodied proprioception (i.e., self-sensing) will become more important to the control of soft robots in unstructured environments. 
In this work, we demonstrate proprioceptive feedback control of a soft, pneumatically-actuated origami robot. 
The robot is a 41 mm long, 3-D printed Kresling-inspired structure with six sets of sidewall folds and one degree of freedom. 
Pneumatic actuation, provided by negative fluidic pressure, causes the robot to contract.
Capacitive sensors patterned onto the robot provide position estimation and serve as input to a feedback controller. 
Using a finite element approach, the electrode shapes were optimized for sensitivity at larger (more obtuse) fold angles to improve control across the actuation range.  
We demonstrate stable position control through a series of contraction set points from 2 mm to 16 mm, with error under 3 mm up to 10 mm contraction. %
Overall, this work contributes optimized capacitive electrode design and the demonstration of closed-loop feedback position control without visual tracking as an input. This approach to capacitance sensing and modeling constitutes a major step towards proprioceptive state estimation and feedback control in soft origami robotics. 



\end{abstract}


\section{Introduction}

Soft robots may soon be part of daily life, with envisioned applications ranging from helping humans \cite{robertson2021soft, wu_stretchable_2021} to holding fragile objects without causing damage \cite{li_vacuum-driven_2019}.
These robots currently have limited impact outside of the lab \cite{hawkes2021hard}. 
A growing body of work is demonstrating the state estimation, position control, and force control \cite{best_new_2016, tapia_makesense_2020} that will be essential for integrating soft robots into these target applications.

A wide range of approaches are used for position or force sensing; common types are motion capture \cite{della_santina_dynamic_2018, patterson_untethered_2020}, pressure sensors external to the actuator \cite{best_new_2016}, and embodied mechanical sensors \cite{yan_origami-based_2023}. 
Many scenarios in which feedback-controlled soft robots are expected to excel over rigid robots, such as collaboration with humans and roles in highly portable applications, present privacy or logistical concerns for motion capture. 
Pressure sensing is only possible for controlling fluidic (pneumatic)  actuators, and its accuracy will vary with leaks and tubing diameter and length. 
Soft mechanical sensors can simultaneously be integrated directly into the robot body and provide accurate force and shape estimations. 
Therefore, improving mechanical sensor performance will be critical to meet future soft robotics sensing and control needs. 

The robot demonstrated in this work is a single degree-of-freedom (DoF) Kresling origami \cite{kresling_origami-structures_2012} robot (Fig. \ref{fig:teaser}a). 
The position of the robot is determined by three sets of capacitive sensors adhered to the robot body.
We chose capacitance as the sensing modality for its high sensitivity, potential for integration into soft fabrication processes, and ability to measure with compact electronics. 
We use fluidic actuation with negative pressure to drive the robot contraction (Fig. \ref{fig:teaser}b). Compared to magnetic field sources or multiple motors to drive cables, our approach offers greater portability and mechanical simplicity as the design contains no internal components. 

\begin{figure}[t]
    \centering
    \includegraphics[width=3.25in]{Figures/IROS_teaser.png}
    \caption{The Kresling robot with (a) capacitive sensors adhered to opposing faces and (b) actuation achieved through negative pressure}
    \label{fig:teaser}
    \vspace{-1.0em}
\end{figure}

This work contributes to the state-of-the-art in soft robotics proprioceptive control by:
\begin{enumerate}
\item designing and optimizing capacitive position sensors using finite element analysis (FEA);
\item programmatically-generating and fabricating the Kresling robot through 3D printing; and 
\item demonstrating feedback control using only the capacitive electrodes. 
\end{enumerate}

Under maximum fluid input, the actuator contraction is 75\% of its extended length (31 mm). 
We demonstrate feedback control to 40\% of the extended length (16 mm), with error below 4 mm for all setpoints. 
To our knowledge, this is the first demonstration of a soft origami robot with feedback control using only capacitive proprioception. 



\section{Related work}

Soft material sensors for actuator shape or force estimation have been demonstrated using flexible circuit components such as capacitors \cite{kim20213d, dorsey2022origami}, resistors \cite{sun_repeated_2022, dong_bioinspired_2022}, or inductors \cite{huang_modular_2022, wang_stick_2022} fixed to the robot body. 
Detecting the angle between two actuator faces has also been well reported \cite{mori_shape-recognizable_2021, wang_stick_2022}, with angle accuracies ranging from 12$^{\circ}$ \cite{mori_shape-recognizable_2021} for a piezoresistive sensor to $\pm$1$^{\circ}$ for an inductive sensor \cite{wang_stick_2022}. 
Fold angle sensing is particularly advantageous in folded and origami robots, where the mechanical properties and deformation of an actuator may be designed through pattern selection and parameters \cite{park_reconfigurable_2022} and the relationship between fold angles and faces is well defined. 

Earlier demonstrations of origami robots folded in paper or polymers focused on the ability to reconfigure, deploy, or self-assemble by folding or unfolding \cite{robertson2021soft, chen_origami_2022} using actuation approaches such as magnetic fields \cite{wu_stretchable_2021,ze_soft_2022}, fluidic pressure \cite{park_reconfigurable_2022,chen_origami_2022}, and tendons \cite{kaufmann_harnessing_2021}.
Insight gained from these fabrication, actuation, and sensing approaches spurred interest in more complex patterns and motions. 
One common design for origami soft robots is the Kresling pattern \cite{kresling_origami-structures_2012, kim_3d_2022, murali_babu_programmable_2023}, due to its ability to achieve bistable states defined by its pattern geometry and its behavior as a revolute joint when compressed.
Prior work has applied the Kresling pattern to create crawlers \cite{ze_soft_2022} and multi-segment continuum arms \cite{kaufmann_harnessing_2021} under magnetic, cable-driven, or fluidic \cite{murali_babu_programmable_2023} actuation. 
The Kresling pattern, and others such as the origami magic ball, have led to demonstrations of grippers \cite{robertson2021soft, wu_stretchable_2021}, crawlers \cite{chen_origami_2022, sun_origami-inspired_2022}, jumpers \cite{sun_repeated_2022}, and haptic feedback devices \cite{williams_4-degree--freedom_2022}.

In contrast to the wealth of soft mechanics and actuator work present in origami robotics literature, position sensing and feedback control research has received less attention.
Notable recent work has investigated the integration of rigid (e.g., photoresistor) or soft mechanical sensors into active origami structures for on-off feedback control. 
Nisser et al. embedded phototransistors and LEDs in a flat origami structure to control angles during structure self-folding \cite{nisser_feedback-controlled_2016}. 
Researchers have also integrated contact switches and tactile sensors \cite{yan_origami-based_2023, sun_origami-inspired_2022} to enable hysteresis control in jumping, gripping, and crawling soft robots.
The uses of soft sensors in this domain include measuring gait and environmental contact in an origami-patterned walker by coating the legs with piezoresistive material \cite{dong_bioinspired_2022}, estimating the curvature of a soft finger with a flexible inductor \cite{huang_modular_2022}, and controlling the fold of a shape memory alloy in three states with a piezoresistive curvature sensor \cite{firouzeh_robogami_2015}. 

\section{Structure and Modeling}

\subsection{Structure and Kinematic Model}
Previous work has thoroughly investigated the mechanics of the Kresling pattern \cite{kaufmann_harnessing_2021, bhovad_peristaltic_2019}. %
Here, we present a short definition of properties relevant to the modeling of the Kresling fold. %
The structure has a single DOF, as described by linked parameters $L$, which is the distance between the top and bottom faces, and $\alpha$, which is the rotation between the faces.
Four parameters control the morphology: the distance between top and bottom faces at full contraction $L_c$, the circumscribing radius around the top face $R$, the angle ratio $\lambda$ between the valley fold and a bottom edge to the angle between a bottom edge and a line that bisects a bottom face inner angle, and the number of Kresling polygon edges $N$. 
The interior angle formed between the center and one edge of the top face is $\phi = \pi/N$. %
Fig. \ref{fig:parameters} represents these parameters on the Kresling structure with views (a) in 2D, looking up through the bottom face, and (b) in 3D.

These variables are linked to one another \cite{kaufmann_harnessing_2021} through 
\begin{equation}
    L = \sqrt{L_c^2 +2R^2\left[ \cos(\alpha + 2 \phi) - \cos (\alpha_c + 2\phi)\right]} ,
    \label{eqn:length}
\end{equation}
where $L$ and $\alpha$ represent a distance and rotation, respectively, between the top and bottom faces, and $\alpha_c$ = 2$\lambda(\pi/2-\phi)$ is the rotation at full contraction. 

We will refer to three additional dependent parameters to describe the Kresling structure.
At full extension, the structure has length $L_e$ and rotation $\alpha_e$.
Two triangular sidewall faces, one with an edge on the top and the other with an edge on the bottom polygon face, intersect to form a valley fold with dihedral angle $\xi$. %

The fold angle $\xi$ is linked to $L$ by finding the angle of intersection between vectors normal to the sidewall triangular faces $n_t$=
\begin{equation}  
\begin{bmatrix}
RL \sin(2\phi) \hat i\\
RL \left( 1 - \cos(2\phi) \right) \hat j\\
R^2 \left( \sin(\alpha)(1-\cos(2 \phi))+(1-\cos(\alpha))(\sin(2 \phi)) \right) \hat k\\
\end{bmatrix}
\end{equation}

and  $n_b$=
{
$\displaystyle$
\begin{equation}
\begin{bmatrix}
RL (\sin(2\phi - \alpha) + \sin(\alpha)) \hat i\\
-RL (\cos(2\phi - \alpha) - \cos(\alpha)) \hat j\\
R^2 \left( (\cos(2\phi - \alpha)-\cos(\alpha))(\sin(2\phi - \alpha)+\sin(2\phi)) \right) \hat k -\\
R^2\left( (\cos(2\phi - \alpha)-\cos(2\phi))(\sin(2\phi - \alpha)+\sin(\alpha)) \right) \hat k\\
\end{bmatrix}
\label{eqn:nvecs}
\end{equation}
}
where $\hat i$, $\hat j$, and $\hat k$ are unit vectors on the axes $x$, $y$, and $z$, respectively, such that 

\begin{equation}
   \cos \xi = \frac{\vec n_t \cdot \vec n_b}{||n_t||||n_b||} . 
   \label{eqn:xi}
\end{equation}
    
We derived the relationship between $L$ and $\xi$ through Eqs. \ref{eqn:length}$-$\ref{eqn:xi}.
Observing that the relationship between fold angle and length is highly linear via a numerical approach ($R^2$ of $99.3\%$ in the range of $L_c$ to $L_e$), we used a linear approximation for the inverse kinematics function $L = 0.22\xi + 10.4$ mm, where $\xi$ is in degrees. 


\begin{figure}[h]
    \centering
    \includegraphics[width=3.25in]{Figures/Kresling_properties.png}
    \caption{The parameters of the Kresling structure (a) from the bottom face looking up and (b) in 3D}
    \label{fig:parameters}
\end{figure}

\subsection{Position Sensors}

Capacitive sensing offers high sensitivity and ease of readout with measurement electronics, making it suitable for displacement sensing in soft robots. 
One potential disadvantage of sensing the pose of the origami robot with capacitors is the relationship between fold angle, electrode distance, and capacitance.
Although the relationship between $\xi$ and $L$ is well approximated with a linear function, the reciprocal relationship between electrode distance and capacitance will yield much lower capacitance at large (more obtuse) fold angles. 
In a Kresling structure where nearly the entire sidewall face is covered with an electrode, these super-linear behaviors will yield a low sensitivity to displacement when the robot is nearly extended.

To obtain a higher sensitivity at larger fold angles, we optimized the electrode shape. 
Due to the lack of closed-form solutions for various electrode shapes, we used FEA (COMSOL v6.0) and a downhill simplex method implemented in MATLAB 
 \cite{lagarias1998convergence} (\texttt{fminsearch}) for optimization.
This approach does not rely on an analytical solution of the gradient (e.g. Newton's method) and was computationally feasible with FEA (e.g., vs. genetic algorithm).
Electrode shapes were represented by five values that control the horizontal and vertical placement of points on the electrode face.
The optimization function was:
\begin{gather}
\text{maximize }f(x) = \frac{\Delta C_{65}(x)}{C_{10}(x)}\end{gather}
where $\Delta C_{65}(x)$ is the capacitance change of a fold moving between 70$\degree$ and 65$\degree$ from a horizontal plane (i.e., $\xi$/2) and is constructed of the vertices in the subset $x$, which is a subset of all potential electrode points in $\mathbb{R}^2$ bounded by the sidewall face. $C_{10}(x)$ is the capacitance at 10$\degree$ also constructed of the same subset vertices $x$.

\begin{figure}[h]
    \centering
    \includegraphics[width=3.25in]{Figures/Optimization.png}
    \caption{Finite element electrode modeling. (a) The initial electrode shapes IC1-IC5 and OC5. The optimized sensitivities are presented in the top left corners.  (b) The simulation results for electrode shapes OC1$-$OC5 and the triangle electrode. \emph{Inset:}  $\Delta C_{65}$.}
    \label{fig:FEA}
\end{figure}

We chose five initial conditions (IC) for the electrode shapes (IC1$-$5) selected from a larger set for variations in initial capacitance and point placement to optimize our electrode shapes (Fig. \ref{fig:FEA}a).
From the optimized electrode (OC) from each initial condition, we selected the electrode with the largest change in capacitance at large fold angle for further testing (i.e., OC5). 
Each minimum fractional sensitivity is presented in Fig. \ref{fig:FEA}a, and the fractional capacitance change ($C-C_{70})/C_{10}$ is presented in Fig. \ref{fig:FEA}b.
The performance of a triangular electrode inset 1.125 mm from the valley fold ($\Delta C_{65}/C_{10}$ of 1.07\%) is also shown. 
Capacitance was also simulated for OC5 across the full range of $\xi$ from extension to contraction.



\section{Fabrication and Experimental Setup}

\subsection{Fabrication}

To create an airtight chamber for fluidic actuation, we 3D printed the robot structure in thermal polyurethane (TPU).
The TPU permits flexibility of the body and the requisite compliance to twist and contract the structure under the negative fluidic pressures that are commonly demonstrated in soft robotics. Moreover, the TPU is sufficiently nonporous, so it maintains a negative vacuum pressure well.
The use of TPU limits the Kresling's stretching at the faces, and we expect its performance to more closely mimic the behavior of paper than that of more extensible soft materials such as silicone rubbers.

Recent work \cite{wu_stretchable_2021, kaufmann_harnessing_2021} has demonstrated Kresling scales from a single millimeter to over 10 centimeters.
Fabrication with a fused deposition modeling 3D printer imposes a practical limit on the scale.
The structure's sidewalls must be sufficiently thin to permit repeated contraction, but thick enough that they are reliably printed without leaks. 
We chose a scale with a visually obvious stroke between fully contracted and extended states of 2 cm or higher. 
Finally, the number of structure edges ($N$) may be four or more. 
However, a trade-off is present between increasing $N$ and the stiffness of the structure, because more faces require more energy to deform the structure folds. 

Taking these factors into account, we fabricated Kresling robots with $N$=6, $R$=3 cm, $L_e$=4.1 cm, wall thickness $t$=1 mm, and $\lambda=0.75$, which all correspond to an $\alpha_e$ of 30$\degree$. %
We set the $\lambda$ value at the midpoint between fully-contracted ($\lambda=0.5$) and fully-extended ($\lambda=1$) values. 
These parameters generate a compliant structure with a maximum extension-contraction stroke of 31 mm.

To fabricate the Kresling robots, we programmatically generated a CAD model of the Kresling structure using a custom script that draws the bottom and sidewall faces given the design variables of $L$, $\alpha_e$, $N$, and $R$ (Fusion 360, Autodesk).
We 3D printed (Creator Pro 2, Flash Forge) the Kresling structure with TPU filament (NinjaFlex Cheetah 95A) (Fig. \ref{fig:fabrication}a). 
Print settings were a 0.4 mm nozzle at an extruder temperature of 238 \degree C, platform temperature of 40 \degree C, layer height of 0.18 mm, and print speed of 30 mms$^{-1}$. 

\begin{figure}[t]
    \centering
    \includegraphics[width=3.25in]{Figures/Fabrication.png}
    \caption{The fabrication steps for the Kresling robot. (a) Additive manufacturing of the robot body, shown halfway. (b) The electrode cut into the target shape with a computer-controlled cutter. (c) The completed robot in the test setup, with a rigid, retroreflective marker plate for optical tracking.}
    \label{fig:fabrication}
\end{figure}

To form the electrodes, we cut copper and nickel plated polyester fabric (Adafruit) into the electrode shape with an electronic cutting machine (Maker 3, Cricut) (Fig. \ref{fig:fabrication}b). %
We adhered these electrodes to opposite faces of the Kresling valley fold to a capacitor. Three capacitors were symmetrically spaced radially around the $z$ axis. 
The placement of the electrodes was guided by extruded lines on the sidewalls.
Each robot takes approximately three hours to print, adhere the electrodes, and seal. 

To actuate and test the robot, we capped the structure with a TPU lid and cyanoacrylate glue (Loctite 495) and inserted pneumatic tubing through holes in the cap. %
Rigid plastic bases were bonded to the top and bottom faces of the Kresling actuator to enforce rigid bodies for kinematics and optical tracking. %
These bases also held the measurement cables at known locations relative to the robot.
Fig. \ref{fig:fabrication}c is a photograph of the robot mounted to a motion capture benchmarking stand.


\subsection{Measurement and Control Setup}

Actuator position was driven by a custom fluidic control board and a set of custom ROS \cite{quigley2009ros} nodes that published capacitance, calculated length, and set pulse width modulation (PWM) values.
A data acquision system (LabJack) sourced a PWM signal to solenoids (Orange Coast Pneumatics) that directly drove fluidic pressure within the Kresling from 101 kPA to 80 kPa absolute. 
Capacitance was read at a rate of 90 Hz with a multi-channel capacitance-to-digital converter (FDC2214 EVM, Texas Instruments). 
Capacitance was measured from three sets of electrodes adhered to alternating sidewalls and averaged for each reading.
Although the Kresling robot has six sets of sidewalls, we were limited to measurement on three sets due to measurement electronics.

The kinematic model was combined with the FEA model of capacitance ($C_{FEA}$) with $\xi$ to estimate the relationship between $L$ and capacitance (Fig. \ref{fig:cap}a).
This relationship was represented in the length calculation function as a third-order polynomial fit. 
Because humidity, local electromagnetic fields, and small variations in electrode placement affect robot capacitance and the match to the FEA model, we mapped $C_{FEA}$ to the measured capacitance as $ C_{meas} = \kappa^{-1}C_{FEA}$, where $\kappa$ is a factor that scales $ C_{meas}$.

After attempting multiple control approaches, including proportional-integral-derivative (PID) and discrete-time control with extensive parameter tuning, we selected discrete-time control due to its high stability and performance in this system. 
The value of the PWM signal at time $t$ that was fed to the solenoid valves on the fluidic control board was 
\begin{equation}
\text{PWM}_t = \text{PWM}_{t-1} + K_p\Delta L + K_d\frac{\Delta L}{\Delta t}
\label{eqn:pwm}
\end{equation}

where PWM$_{t-1}$ is the PWM value of the previous time step, $K_p$ is the proportional gain constant, $K_d$ is the derivative gain constant, $\Delta L$ is the error between the setpoint and the measured contraction, and $\Delta t$ is the time step.
The proportional and derivative gain values were tuned by hand with values of 0.005 and 0.001, respectively. 
The center of mass position and rotation of the actuator were measured using a commercial motion capture system (V120:Trio, OptiTrack) and served as the ground truth. %


\section{Results}


\subsection{Open-loop Characterization}

We fabricated and compared the sensitivity of electrode OC5 and the triangular electrode by placing one set of each electrode type on the sidewalls of the same Kresling.  
We performed 12 cycles between 0 mm and 17 mm of contraction 
Because we cannot directly track fold angle through the motion capture system, we present the following results in terms of robot contraction.

The capacitance change per area between 0 mm and 17 mm of contraction is 0.22 pFcm$^{-2}$ and 0.61 pFcm$^{-2}$ for the triangular and optimized electrodes, respectively. 
While the absolute sensitivity of the triangular electrode is higher, the optimized electrodes yield 2.8 times higher capacitance per unit area.   

After cyclic testing, we examined the electrodes for physical degradation. %
The optimized electrodes, which sit in the center of the sidewall, showed no delamination from the robot body (Fig. \ref{fig:cyclic_electrodes}b) when compared to the pre-test condition (Fig. \ref{fig:teaser}a). 
In contrast, the triangular electrodes wrinkled and delaminated at the corners (Fig. \ref{fig:cyclic_electrodes}c).  
This delamination was deemed unacceptable because loose electrodes may contact during contraction and yield inaccurate measurements. Therefore, the following tests are presented only with the optimized electrodes. 

A Kresling robot with three sets of electrodes (S0, S1, and S2) symmetrically placed around the robot on the sidewall folds was fabricated and actuated to 17 mm contraction over 90 seconds.
Fig. \ref{fig:cap}a shows the relationship between measured $\alpha$ and $\alpha$ estimated from the actuator length over this contraction. The root mean square error (RMSE) between measured $\alpha$ and kinematic model $\alpha$ is 1.5$\degree$.
Fig. \ref{fig:cap}b demonstrates $C_{meas}$ for each electrode set, and the average across all three electrode sets, alongside $C_{FEA}$. 
The scale factor $\kappa$ fit to these data is 0.26.

\begin{figure}[h]
    \centering
    \includegraphics[width=3.25in]{Figures/Openloop.png}
    \caption{Open-loop response with contraction. (a) Measured and kinematic model of top face rotation $\alpha$. (b) FEA and measured capacitance change, which is zero at the fully-extended length.}
    \label{fig:cap}
\end{figure}



\subsection{Feedback Control}

The setpoint was stepped from full extension to a contracted value under feedback control according to (\ref{eqn:pwm}). 
The response of the Kresling robot to multiple commanded setpoints  is shown in Fig. \ref{fig:feedback}a, including at setpoints of 18 mm, 12 mm, and 6 mm (Fig. \ref{fig:feedback}a-b), the average length across three trials and RMSE from setpoint across three trials (Fig. \ref{fig:feedback}c), and for time-varying sinusoidal and stepped control setpoints (Fig. \ref{fig:feedback}d-e). 
RMSE and length are calculated from 20 s to 90 s during the test, and the errorbars in Fig. \ref{fig:feedback}c represent standard deviation in length over three tests.


\section{Discussion}

The Kresling structure offers a rich testbed for investigating sensor performance in a soft robot. 
Integration of capacitive sensors onto the Kresling body permitted position control for contraction setpoints up to 17 mm, or 41\% of the total robot length, with RMSE below 3 mm for setpoints less than 10 mm and below 4 mm for all setpoints.
One source of error was the mapping from capacitance to length. 
The linear relationship observed in Fig. \ref{fig:feedback}c between length and setpoint has a slope higher than one, or a higher estimate of position. Decreasing scale factor $\kappa$ may improve position estimation. 

We demonstrated that the non-optimized triangle electrode had higher sensitivity, but it was not robust to repeated actuation. 
We attribute this performance to the mismatch between electrode strain and Kresling strain, particularly at the corners. 
The actuator visibly twists and stretches, causing the inextensible electrodes to delaminate. 
The optimized electrodes are placed on sidewalls that remain relatively planar and unstretched, with only small concavity when a vacuum is introduced. 
This reduced extension reduces the likelihood of delamination.

\begin{figure}[H]
    \centering
    \includegraphics[width = 3.25in]{Figures/Feedback.png}
    \caption{Feedback control response. (a) Three setpoints over 10 s and (b) over 90 s. (c) The actuator length across three trials and RMSE. (d) The response to a commanded sinusoidal input and (e) multiple control input steps. }
    \label{fig:feedback}
\end{figure}

Increasing setpoint beyond 17 mm of contraction caused instability, which is visible in Fig. \ref{fig:feedback}a as rapid oscillation around the setpoint. 
At this distance, the known bistable properties of the Kresling structure cause the robot to rapidly undergo a change in state that the controller cannot compensate for. 
Overshooting the setpoint causes the electrodes to make momentary contact, which results in near-zero capacitance readings due to the output of the measurement electronics and therefore erroneously calculated short lengths. 
The system overcompensates as it perceives a much larger error than is present. 
This behavior is present in the first few seconds of the sinusoid in Fig.~\ref{fig:feedback}e.
It shows the ability to follow a cyclic pattern; however, at larger contraction amplitudes, the system must overcome both the elastic restoring force present when the Kresling contracts to reach the set point and generates overshoot. 
To avoid this error in practice, we can simply restrict the contraction range of the contraction below the point of bi-stability, thus preventing rapid change, overshoot, and contact.  

The nonlinear capacitance-length relationship, non-rigid deformation, and bi-stable behavior add complexity to feedback control and provide additional motivation for feedback control over open-loop control.
While open-loop control is more common in soft robotics, it also requires a much finer degree of system identification for accurate control. 
Therefore, we view proprioceptive feedback as a crucial capability for emerging soft robotics. 







\section{Conclusions}
Applying proprioceptive position sensing to control actuator position is an ongoing challenge in soft robotics. 
To address this challenging problem, we demonstrated a Kresling-inspired, 3D printed, fluidically actuated robot with capacitive sensors integrated onto the sidewall faces. 
Through optimizing the geometry of the capacitive electrodes, we maximized the sensitivity at large-fold angles.
We further demonstrated the ability to transition between setpoint states, achieved less than 4 mm setpoint error across a setpoint to 17 mm, and explored complex motion patterns such as tracking a sine wave. 
We are actively investigating extensions of this work to multi-DOF origami actuators. 
Joining several of these enhanced Kresling structures will enable complex motion strategies that include crawling and movement in 6-DOF pose space. 
Other areas of future work include improving the electrode design and fabrication approach to reduce capacitance variations between electrode pairs and investigating different control approaches. 

The results of this work demonstrate that capacitive sensing is a promising technique for proprioceptive state estimation in soft robotics.


\section*{Acknowledgements}
The authors thank A. Allison, S. Alt, and G. Lvov for assistance with experimental setup and 3D printing, and T. Padir for use of the Optitrack system.













